Deep follow-up for gravitational-wave inference: a case study with GW151226

New analyses of gravitational wave events raise questions about the nature of some events. For example, LIGO--Virgo--KAGRA initially determined GW151226 to be a merger with a mass-ratio $q\approx0.5$ and effective inspiral spin $\chi_{\text{eff}}\approx 0.2$. However, recent works offer an alternative picture: GW151226 is a lower-mass-ratio event $q \approx 0.3$ with slightly higher spin $\chi_{\text{eff}}\approx 0.3$. This discrepancy has been challenging to resolve as a wide range of differences are employed for each analysis. This work introduces a ``deep follow-up'' framework to efficiently compute the posterior odds between two different peaks in parameter space. In doing so, we aim to help resolve disputes about the true nature of gravitational-wave events associated with conflicting astrophysical interpretations. Our proposal is not a replacement for standard inference techniques; instead, our method provides a diagnostic tool to understand discrepancies between conflicting results. We demonstrate this method by studying three {$q$-$\chi_{\text{eff}}$} peaks proposed for GW151226. We find the $(q\sim0.5, \chi_{\text{eff}}\sim0.2)$ interpretation is only slightly preferred over the $(q\sim0.3, \chi_{\text{eff}}\sim0.3)$ hypothesis with a posterior odds of $\sim1.7\pm0.4$, suggesting that neither of the two peaks can be ruled out. We discuss strategies to produce more reliable parameter estimation studies in gravitational-wave astronomy.

==> Deep follow-up of GW151226_ ordinary binary or extreme mass ratio system_/custom_commands.tex <==


\newcommand{\qxeffPt}{\vec{\mu}}
\newcommand{\fancytext}[1]{{\relax\ifmmode#1\else $#1$\fi}\xspace}
\newcommand{\mathcmd}[1]{{\sc \relax\ifmmode#1\else $#1$\fi}\xspace}
\newcommand{\xp}{\mathcmd{\chi_{\text{p}}}}
\newcommand{\xeff}{\mathcmd{\chi_{\text{eff}}}}

\newcommand{\odds}{\mathcmd{\mathcal{O}^{\rm A}_{\rm B}}}
\newcommand{\kdeodds}{\mathcmd{{}^{K}\mathcal{O}^{\rm A}_{\rm B}}}

\newcommand{\avi}[1]{\textcolor{orange}{[Avi: #1]}}


\newcommand{\SPA}{School of Physics and Astronomy, Monash University, VIC 3800, Australia}
\newcommand{\OzGravMonash}{OzGrav: The ARC Centre of Excellence for Gravitational Wave Discovery, Monash University, VIC 3800, Australia}

\newcommand{\chia}{Chia \textit{et al.}}
\newcommand{\mateu}{Mateu-Lucena \textit{et al.}}
\newcommand{\nitz}{Nitz \textit{et al.}}

\newcommand{\chiap}{Chia${}_{+}$}
\newcommand{\mateup}{ML${}_{+}$}
\newcommand{\nitzp}{Nitz${}_{+}$}


\newcommand{\kdeMvC}{{}^K\mathcal{O}^{\rm \mateup}_{\rm \chiap}}
\newcommand{\kdeMvN}{{}^K\mathcal{O}^{\rm \mateup}_{\rm \nitzp}}


\newcommand{\code}[1]{{\texttt{#1}}\xspace}
\newcommand{\bilby}{\code{bilby}}
\newcommand{\parallelbilby}{\code{parallel-bilby}}
\newcommand{\gwpop}{\code{GWPopulation}}
\newcommand{\bilbypipe}{\code{bilby-pipe}}
\newcommand{\dynesty}{\code{dynesty}}
\newcommand{\imrphenomxphm}{\texttt{IMRPhenomXPHM}}


\BeforeBegin{NiceTabular}{\let\begin\BeginEnvironment\let\end\EndEnvironment}
\BeforeBegin{NiceArray}{\let\begin\BeginEnvironment}
\BeforeBegin{NiceMatrix}{\let\begin\BeginEnvironment}


%%%%%%%%%%%%%%%%%%%%%
% Nitz+: q ${0.53}_{-0.23}^{+0.24}$, xeff ${0.22}_{-0.06}^{+0.10}$
% Mateu+: q ${0.52}_{-0.21}^{+0.27}$, xeff ${0.20}_{-0.06}^{+0.10}$
% Chia+: q ${0.30}_{-0.13}^{+0.22}$, xeff ${0.30}_{-0.11}^{+0.17}$
\newcommand{\qMateu}{\mathcmd{{0.52}_{-0.21}^{+0.27}}}
\newcommand{\xeffMateu}{\mathcmd{{0.20}_{-0.06}^{+0.10}}}
\newcommand{\qChia}{\mathcmd{{0.30}_{-0.13}^{+0.22}}}
\newcommand{\xeffChia}{\mathcmd{{0.30}_{-0.11}^{+0.17}}}
\newcommand{\qNitz}{\mathcmd{{0.53}_{-0.23}^{+0.24}}}
\newcommand{\xeffNitz}{\mathcmd{{0.22}_{-0.06}^{+0.10}}}
%%%%%%%%%%%%%%%%%%%%%





% Pts                     KDE Post Odds  Prior Odds     Bayes Factor  'Deep' Post Odds
% GW151226 Mateu Vs Chia  3.47+/-0.13    1.674+/-0.010  1.00+/-0.21   1.7+/-0.4
% GW151226 Mateu Vs Nitz  1.46+/-0.04    1.076+/-0.011  1.31+/-0.21   1.41+/-0.29




% -----------------------  -------------  -------------  ------------  ----------------
% Pts                      KDE Post Odds  Prior Odds     Bayes Factor  'Deep' Post Odds
% KDE-Mateu Mateu VS Chia  3.45+/-0.14    1.677+/-0.013  1.00+/-0.21   1.7+/-0.4
% KDE-Chia Mateu VS Chia   0.328+/-0.004  1.676+/-0.012  1.00+/-0.21   1.7+/-0.4
% KDE-Nitz Mateu VS Chia   1.715+/-0.014  1.676+/-0.012  1.00+/-0.21   1.7+/-0.4
% -----------------------  -------------  -------------  ------------  ----------------
\newcommand{\MkdeMvC}{\mathcmd{3.45\pm0.01}}
\newcommand{\CkdeMvC}{\mathcmd{0.33\pm0.01}}
\newcommand{\NkdeMvC}{\mathcmd{1.72\pm0.01}}
\newcommand{\priMvC}{\mathcmd{1.68\pm0.01}}
\newcommand{\bfMvC}{\mathcmd{1.0\pm0.2}}
\newcommand{\deepOMvC}{\mathcmd{1.7\pm0.4}}


% -----------------------  -------------  -------------  ------------  ----------------
% Pts                      KDE Post Odds  Prior Odds     Bayes Factor  'Deep' Post Odds
% KDE-Mateu Mateu VS Nitz  1.46+/-0.04    1.076+/-0.011  1.31+/-0.21   1.42+/-0.29
% KDE-Chia Mateu VS Nitz   0.927+/-0.011  1.076+/-0.010  1.31+/-0.21   1.42+/-0.29
% KDE-Nitz Mateu VS Nitz   0.870+/-0.006  1.076+/-0.012  1.31+/-0.21   1.41+/-0.29
% -----------------------  -------------  -------------  ------------  ----------------
\newcommand{\MkdeMvN}{\mathcmd{1.46\pm0.04}}
\newcommand{\CkdeMvN}{\mathcmd{0.93\pm0.01}}
\newcommand{\NkdeMvN}{\mathcmd{0.87\pm0.01}}
\newcommand{\priMvN}{\mathcmd{1.08\pm0.01}}
\newcommand{\bfMvN}{\mathcmd{1.3\pm0.2}}
\newcommand{\deepOMvN}{\mathcmd{1.4\pm0.3}}

% ----------------------  -------------  -------------  ------------  ----------------
% Pts                     KDE Post Odds  Prior Odds     Bayes Factor  'Deep' Post Odds
% KDE-Mateu Nitz VS Chia  2.38+/-0.10    1.560+/-0.012  0.76+/-0.21   1.19+/-0.25
% KDE-Chia Nitz VS Chia   0.355+/-0.004  1.556+/-0.011  0.76+/-0.21   1.18+/-0.25
% KDE-Nitz Nitz VS Chia   1.973+/-0.014  1.556+/-0.011  0.76+/-0.21   1.18+/-0.25
% ----------------------  -------------  -------------  ------------  ----------------
\newcommand{\MkdeNvC}{\mathcmd{2.38\pm0.1}}
\newcommand{\CkdeNvC}{\mathcmd{0.36\pm0.01}}
\newcommand{\NkdeNvC}{\mathcmd{1.97\pm0.01}}
\newcommand{\priNvC}{\mathcmd{1.56\pm0.01}}
\newcommand{\bfNvC}{\mathcmd{0.8\pm0.2}}
\newcommand{\deepONvC}{\mathcmd{1.2\pm0.3}}


%%% OLD VALUES
\newcommand{\oddsVal}{1.2}
\newcommand{\kdeoddsVal}{7.5}
\newcommand{\bfVal}{0.3}
\newcommand{\prioroddsVal}{4.2}


% colors
\definecolor{OliveGreen}{rgb}{0,0.6,0}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}

\newcommand{\newtxt}[1]{#1} % {\green{#1}}
\newcommand{\deltxt}[1]{\st{\red{#1}}}


\newenvironment{sectionNew}[1]
  {\section[#1]{\textcolor{OliveGreen}{#1}}\color{OliveGreen}}
  {\normalcolor}
\newenvironment{subsectionNew}[1]
  {\subsection[#1]{\textcolor{v}{#1}}\color{OliveGreen}}
  {\normalcolor}
\newenvironment{sectionFinished}[1]
  {\section[#1]{\textcolor{black}{#1}}\color{black}}
  {\normalcolor}
\let\endsection\relax
\let\endsubsection\relax
